Entanglement Negativity at Measurement-Induced Criticality

We propose entanglement negativity as a fine-grained probe of measurement-induced criticality. We motivate this proposal in stabilizer states, where for two disjoint subregions, comparing their "mutual negativity" and their mutual information leads to a precise distinction between bipartite and multipartite entanglement. In a measurement-only stabilizer circuit that maps exactly to two-dimensional critical percolation, we show that the mutual information and the mutual negativity are governed by boundary conformal fields of different scaling dimensions at long distances. We then consider a class of "hybrid" circuit models obtained by perturbing the measurement-only circuit with unitary gates of progressive levels of complexity. While other critical exponents vary appreciably for different choices of unitary gate ensembles at their respective critical points, the mutual negativity has scaling dimension 3 across remarkably many of the hybrid circuits, which is notably different from that in percolation. We contrast our results with limiting cases where a geometrical minimal-cut picture is available.

==> K_struct.tex <==
\begin{tikzpicture}[scale = 0.5,every node/.style={scale = 0.75}]
  \begin{scope}[shift={(0,2)}]
    \draw[dashed] (0,0) rectangle (2,2);
    \draw[dashed] (0,1)--(2,1);
    \draw[dashed] (1,0)--(1,2);
    \node () at (0.5,0.5) {$\mathbb{I}$};
    \node () at (0.5,1.5) {$0$};
    \node () at (1.5,1.5) {$\mathbb{I}$};
    \node () at (1.5,0.5) {$0$};
    \draw [decorate,decoration={brace,amplitude=2pt,raise=0pt,mirror},yshift=0pt]
    (0+0.05,-0.2) -- ++(0.9,0) node [black,midway,xshift=0pt,yshift=-10pt] {\small $k_A$};
  \end{scope}
  \draw[dashed] (0,0) rectangle (4,4);
  \draw[dashed] (0,1)--++(3,0)--++(0,3);
  \draw[dashed] (2,2)--++(1,0);
  \draw[dashed] (2,2)--++(0,-1);
  \draw[dashed] (3,1)--++(1,0);
  \draw[dashed] (3,1)--++(0,-1);
  \node () at (2.5,1.5) {$0$};
  \node () at (3.5,0.5) {$0$};
  \draw [decorate,decoration={brace,amplitude=2pt,raise=0pt,mirror},yshift=0pt]
  (0+0.05,1-0.2) -- ++(3-0.1,0) node [black,midway,xshift=0pt,yshift=-10pt] {\small $m_A$};
  \draw [decorate,decoration={brace,amplitude=2pt,raise=0pt},yshift=0pt]
  (2+0.05,2+0.2) -- ++(1-0.1,0) node [black,midway,xshift=0pt,yshift=10pt] {\small $\mu_A$};
  \draw [decorate,decoration={brace,amplitude=2pt,raise=0pt,mirror},yshift=0pt]
  (0+0.05,-0.2) -- ++(4-0.1,0) node [black,midway,xshift=0pt,yshift=-10pt] {\small $m$};
  \draw[line width = 1pt] (-0.1,-0.5)--++(-0.2,0)--++(0,4.7)--++(0.2,0);
  \draw[line width = 1pt] (4.1,-0.5)--++(0.2,0)--++(0,4.7)--++(-0.2,0);
  % \draw[dashed, red] (2,1) rectangle (3,2);
  % \draw[dashed, blue] (3,0) rectangle (4,1);
  \draw[dashed, red] (1,1) rectangle (3,3);
\end{tikzpicture}

==> app_CPLC_configs.tex <==
\section{More figures on CPLC configurations}

{
Here I am including some typical configurations of the CPLC, for fun.
Will delete eventually.
}

In Fig.~\ref{fig:loop_figs_limit_0}, I plot the case for $p = 0$ (no crossing, Sec.~\ref{sec:moc_majorana}), which is percolation.
There are two insulating phases and a critical point.

In Fig.~\ref{fig:loop_figs_limit_3}, I plot points in the insulating phase at $p = 0.3$ (weak crossing) and $q = 0, 1$.
The bulk contains a lot of short loops despite crossing, and we see an edge mode is present at $q = 1$ but absent at $q = 0$, as expected from the $p = 0$ limit.


In Fig.~\ref{fig:loop_figs_limit_5}, I plot points in the insulating phase at $p = 0.5$ (slightly stronger crossing) and $q = 0, 1$.
This is similar to Fig.~\ref{fig:loop_figs_limit_3}, except when $p = 0.5, q = 0$, we see that the typical size of an \emph{edge connected component} grows due to increased crossing.


In Fig.~\ref{fig:loop_figs_limit_9}, I plot points in the insulating phase at $p = 0.9$ (very strong crossing) and $q = 0, 1$.
The edge connected component is already larger than the system size, and we cannot really tell between $q=0$ and $q=1$.
However, in the thermodynamic limit, only the $q=1$ point should have an infinite edge mode.
Also, the bulk already looks pretty metallic.

In Fig.~\ref{fig:loop_figs_metal_a}, I plot points in the metallic phase at $(p,q) = (0.5,0.5)$ and $(p,q) = (0.9,0.5)$.
Both have very few short loops in the bulk, and a seemingly edge connected component of infinite size.
{
This does not immediately contradict the loop size distribution in Eq.~\eqref{eq:P_arc_CPLC},
\env{align}{
    P_{\rm arc}(\ell) \propto \(\ln \ell\) \ell^{-2},
}
since now I am joining the the Majorana arcs at each qubit, which can possibly lead to an arc of infinite size.
}


In Fig.~\ref{fig:loop_figs_metal_b}, I plot a few more points in the metallic phase long the $q=0.5$ line at $p = 0.2, 0.4, 0.6, 0.8$.
This is similar to Fig.~\ref{fig:loop_figs_metal_a}, but now we can see how crossing increases the typical size of a ``slab'' (square lattice like region) in the bulk, which diverges as $p \to 1$.

In Fig.\ref{fig:loop_figs_metal_c}, I plot two more points in the metallic phase close to the critical lines.
Here, it seems that both can still have an infinite-sized edge connected component.


In Fig.\ref{fig:loop_figs_critical}, I plot two points on the critical lines.
At the transition to the trivial insulator $(p = 0.5, q=0.1770)$, the edge connectivity seems reduced (it seems to have broken in parts) as compared to Fig.~\ref{fig:loop_figs_metal_c}.

{
Here is a guess: we see the ``normal'' exponent $h_{\rm MN} \approx 3.0$ as we move within the metallic phase and at the transition to the topological insulator, because there is no change in the edge topology (we always have an edge mode).
However, at the transition to trivial insulator, the number of edge modes jumps from $1$ to $0$, and this is why we see the anomalous exponent $h_{\rm MN} \approx 2.5$.
Just a guess.
}


%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{loop_figs/limit/p_0.0000_q_0.0000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/limit/p_0.0000_q_1.0000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/critical/p_0.0000_q_0.5000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/limit/p_1.0000_q_0.0000.pdf}
    \caption{{No crossings (percolation).} (Left) $(p,q) = (0,0)$; (Right) $(p,q) = (0,1)$; (Lower left) $(p, q) = (0,0.5)$.\\
    (Lower right) {\red Crossing only.} $(p, q) = (1,0)$.
    }
    \label{fig:loop_figs_limit_0}
\end{figure}
%-------------------------------------------------

%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.3000_q_0.0000_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.3000_q_1.0000_L.pdf}
    \caption{{Insulators.} (Upper) $(p,q) = (0.3,0)$; (Lower) $(p,q) = (0.3,1)$.
    }
    \label{fig:loop_figs_limit_3}
\end{figure}
%-------------------------------------------------

%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.5000_q_0.0000_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.5000_q_1.0000_L.pdf}
    \caption{{Insulators.} (Upper) $(p,q) = (0.5,0)$; (Lower) $(p,q) = (0.5,1)$.
    }
    \label{fig:loop_figs_limit_5}
\end{figure}
%-------------------------------------------------


%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.9000_q_0.0000_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/limit/p_0.9000_q_1.0000_L.pdf}
    \caption{{Insulators.} (Upper) $(p,q) = (0.9,0)$; (Lower) $(p,q) = (0.9,1)$.
    }
    \label{fig:loop_figs_limit_9}
\end{figure}
%-------------------------------------------------


%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/metal/p_0.5000_q_0.5000_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/metal/p_0.9000_q_0.5000_L.pdf}
    \caption{{Metals.} (Upper) $(p,q) = (0.5,0.5)$; (Lower) $(p,q) = (0.9,0.5)$.
    }
    \label{fig:loop_figs_metal_a}
\end{figure}
%-------------------------------------------------

%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{loop_figs/metal/p_0.2000_q_0.5000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/metal/p_0.4000_q_0.5000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/metal/p_0.6000_q_0.5000.pdf}
    \includegraphics[width=.45\textwidth]{loop_figs/metal/p_0.8000_q_0.5000.pdf}
    \caption{{Metals.} (Upper left) $(p,q) = (0.2,0.5)$; (Upper right) $(p,q) = (0.4,0.5)$; (Lower left) $(p,q) = (0.6,0.5)$; (Lower right) $(p,q) = (0.8,0.5)$.
    }
    \label{fig:loop_figs_metal_b}
\end{figure}
%-------------------------------------------------


%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/metal/p_0.5000_q_0.2000_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/metal/p_0.5000_q_0.8000_L.pdf}
    \caption{{Metals.} (Upper) $(p,q) = (0.5,0.2)$; (Lower) $(p,q) = (0.5,0.8)$.
    }
    \label{fig:loop_figs_metal_c}
\end{figure}
%-------------------------------------------------


%-------------------------------------------------
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{loop_figs/critical/p_0.5000_q_0.1770_L.pdf}
    \includegraphics[width=.7\textwidth]{loop_figs/critical/p_0.5000_q_0.8230_L.pdf}
    \caption{{Critical points.} (Upper) $(p,q) = (0.5,0.1770)$; (Lower) $(p,q) = (0.5,0.8230)$.
    }
    \label{fig:loop_figs_critical}
\end{figure}
%-------------------------------------------------

==> app_EN_stab_v1.tex <==
\section{Entanglement negativity (EN) of stabilizer states : more details\label{app:EN_stab}}

%\subsection{$\mc{N}_A(\rho_Q(\mc{S})) = \frac{1}{2} \dim \mathrm{Im}(\mathsf{K}_A)$}


\subsection{An algorithm for computing EN}

Let $A$ and $B$ each be a set of % $|Q|$
qubits, $\mc{S}$ be an abelian subgroup of the Pauli group $\mc{P}(A \cup B)$, and $\mc{G}(\mc{S})$ be a linearly independent generating set (or simply a ``basis'') of $\mc{S}$.
We have
\env{align}{
    \mc{G}(\mc{S}) =&\, \{g_1, \ldots g_{|\mc{G}(\mc{S})|} \}, \\
    \mc{S} =&\, \avg{\mc{G}(\mc{S})}, \quad \dim \mc{S} = \lv \mc{G}(\mc{S}) \rv = \log_2 \lv \mc{S} \rv.
}
Here $\dim \mc{S}$ is the dimension of $\mc{S}$ when viewed as a vector space.
We will henceforth denote
\env{align}{
    m \coloneqq \dim \mc{S} = \lv \mc{G}(\mc{S}) \rv = \log_2 \lv \mc{S} \rv.
}

The subgroup $\mc{S}$ defines the following physical density matrix on ${A \cup B}$,
\env{align}{
    \rho_{A \cup B}= \frac{1}{2^{|{A \cup B}|}} \sum_{g \in \mc{S}} g.
}


Given the bipartition $(A,B)$ of $A \cup B$, we define the following mappings
\env{itemize}{
\item
The ``restriction'' on $A$:
\env{align}{
    \mathrm{proj}_A : \hspace{.3in} \mc{P}(A \cup B) \quad \to&\quad \mc{P}(A) \nn
    g_A \otimes g_B \quad \mapsto&\quad g_A
}
\item
The ``partial transpose'' on $A$:
\env{align}{
    \Gamma_A : \hspace{.3in} \mc{P}(A \cup B) \quad \to&\quad \mc{P}(A \cup B) \nn
    g_A \otimes g_B \quad \mapsto&\quad (g_A)^\mathsf{T} \otimes g_B
}
Here $\mathsf{T}$ denotes the matrix transposition, say in the computational basis where
\env{align}{
    X = \env{pmatrix}{
        0 & +1\\
        +1 & 0
    }, \quad 
    Y = \env{pmatrix}{
        0 & -i\\
        +i & 0
    }, \quad 
    Z = \env{pmatrix}{
        +1 & 0\\
        0 & -1
    }.
}
}
The partial transpose of $\rho_{A \cup B}$ is as follows
\env{align}{
    \rho_{A \cup B}^{\Gamma_A} = 
    \frac{1}{2^{|{A \cup B}|}} \sum_{g \in \mc{S}} g^{\Gamma_A}.
}


Since $X^\mathsf{T} = X$, $Z^\mathsf{T} = Z$, while $Y^\mathsf{T} = -Y$,
the partial transpose introduces a factor $x_A(g) \coloneqq (-1)^{\#Y_A(g)}$ on $g \in \mc{P}({A \cup B})$, where $\#Y_A(g)$ counts the number of $Y$ factors in $\mathrm{proj}_A(g)$,
\env{align}{
    g^{\Gamma_A} = (-1)^{\#Y_A(g)} g = x_A(g) \cdot g.
}
Define a sign function $\mathrm{Sgn}_A (g, h) \in \{-1, +1\}$, such that 
\env{align}{
    \mathrm{proj}_A(g) \cdot \mathrm{proj}_A(h) = \mathrm{Sgn}_A(g, h)\,  \mathrm{proj}_A(h) \cdot \mathrm{proj}_A(g).
}
A key observation is the following ``cocycle condition'', that can be explicitly verified:
\env{align}{
    x_A(g) x_A(h) x_A(gh) = \mathrm{Sgn}_A (g, h).
}

Let us also define the following $m \times m$ ``commutator matrix'',
\env{align}{
    \(\mathsf{K}_A\)_{ij} = \env{cases}{
        0, \text{ if } \mathrm{proj}_A(g_i) \cdot \mathrm{proj}_A(g_j) = + \mathrm{proj}_A(g_j) \cdot \mathrm{proj}_A(g_i) \\
        1, \text{ if } \mathrm{proj}_A(g_i) \cdot \mathrm{proj}_A(g_j) = - \mathrm{proj}_A(g_j) \cdot \mathrm{proj}_A(g_i)
    }
    %\text{ for } 1 \le i, j \le m,
}
for $1 \le i, j \le m$,
where the $g_i$'s on the RHS are elements of $\mc{G}(\mc{S})$.
It is obvious that $\mathsf{K}_A$ is symmetric, and has $0$'s on its diagonal.

For an arbitrary element $g \in \mc{S}$, we have the following representation
\env{align}{
    g \coloneqq g^u = \prod_{j = 1}^m g_j^{u_j},  \text{ where } u \in \{0, 1\}^{m} = \(\mathbb{F}_2\)^m, g_j \in \mc{G}(\mc{S}).
}
We then have
\env{align}{
    \mathrm{Sgn}_A(g^u, g^v) = (-1)^{\avg{u, \mathsf{K}_A v}}.
}


With these, we want to show that $\( \rho_{A \cup B}^{\Gamma_A} \)^2 \propto \( \rho_{A \cup B}^{\Gamma_A} \)^4$.
\env{align}{
    & \( \rho_{A \cup B}^{\Gamma_A} \)^2 \nn
    =& 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} g^{\Gamma_A} h^{\Gamma_A} \nn
    =& 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} x_A(g) x_A(h) \cdot gh \nn
    =& 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} x_A(g) x_A(gh) \cdot h \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} \mathrm{Sgn}_A (g, h) x_A(h) \cdot h \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{u, v \in \(\mathbb{F}_2\)^m} \mathrm{Sgn}_A (g^u, g^v) x_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{v \in \(\mathbb{F}_2\)^m} \( \sum_{u \in \(\mathbb{F}_2\)^m} (-1)^{\avg{u, \mathsf{K}_A v}} \) x_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{v \in \(\mathbb{F}_2\)^m} 2^m \cdot \delta(\mathsf{K}_A v, \mathbf{0}) \cdot x_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|-m}} \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)} x_A(g^v) \cdot g^v,
}
\env{align}{
    & \( \rho_{A \cup B}^{\Gamma_A} \)^4 \nn
    =&
    \lz
    \frac{1}{2^{2|{A \cup B}|-m}} \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)} x_A(g^v) \cdot g^v
    \rz^2 \nn
    =&
    \frac{1}{2^{4|{A \cup B}|-2m}} \sum_{u, v \in \mathrm{Ker}(\mathsf{K}_A)} x_A(g^u) x_A(g^v) \cdot g^u g^v
    \nn
    =&
    \frac{1}{2^{4|{A \cup B}|-2m}} \sum_{u, v \in \mathrm{Ker}(\mathsf{K}_A)} (-1)^{\avg{u, \mathsf{K}_A(v)}} x_A(g^{u+v})  \cdot g^{u+v}
    \nn
    =&
    \frac{1}{2^{4|{A \cup B}|-2m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)}  x_A(g^{v})  \cdot g^{v}
    \nn
    =&
    \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv \( \rho_{A \cup B}^{\Gamma_A} \)^2.
}
Thus,
\env{align}{
    %& (\ln 2)^{-1} \mc{N}(\rho) \nn
    & (\ln 2)^{-1} N_A(\rho_{A \cup B}) \nn
    =& \lim_{n\to \frac{1}{2}} \log_2 \mathrm{Tr} \( \rho_{A \cup B}^{\Gamma_A} \)^{2n} \nn
    =& \lim_{n\to \frac{1}{2}} \log_2 \ld
    \( \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv\)^{n-1}
    \mathrm{Tr} \( \rho_{A \cup B}^{\Gamma_A} \)^2
    \rd \nn
    =& \lim_{n\to \frac{1}{2}} \log_2 \ld
    \( \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv\)^{n-1}
    \frac{1}{2^{|{A \cup B}|-m}}
    \rd \nn
    =& \log_2 \( \frac{2^m}{\lv \mathrm{Ker}(\mathsf{K}_A) \rv}\)^{1/2} \nn
    =&\,
    \frac{1}{2} \lz m - \dim \mathrm{Ker}(\mathsf{K}_A) \rz \nn
    =&\,
    \frac{1}{2} \dim \mathrm{Im}(\mathsf{K}_A). % \nn
    % =&\,
    % \frac{1}{2} \mathrm{rank}(\mathsf{K}_A).
}
It is perhaps obvious that 
\env{align}{
N_A(\rho_{A \cup B}) = N_B(\rho_{A \cup B}),
}
since $\mathsf{K}_A = \mathsf{K}_B$.
This is indeed consistent with
\env{align}{
    \(\rho_{A \cup B}^{\Gamma_A}\)^{\mathsf{T}} = \rho_{A \cup B}^{\Gamma_{A \cup B}}.
}




%Next we try to characterize $\mc{N}_A(\rho_Q(\mc{S})) = \frac{1}{2} \dim \mathrm{Im}(\mathsf{K}_A)$.

%\subsection{$\dim \mathrm{Im}(\mathsf{K}_A) = \dim \mathrm{proj}_A (\mc{S}) - \dim Z(\mathrm{proj}_A (\mc{S}))$}

\subsection{EN from the stabilizer group}

%Let $\mc{G}(\mathrm{proj}_A(\mc{S}))$ be a basis of $\mathrm{proj}_A(\mc{S})$, and define
Define
\env{align}{
    m_A \coloneqq \dim \mathrm{proj}_A (\mc{S}) % = \lv \mc{G}(\mathrm{proj}_A(\mc{S})) \rv = \log_2 \lv \mathrm{proj}_A(\mc{S}) \rv
    \le m.
}
Without loss of generality, we assume
\env{align}{
    \mathrm{proj}_A(\mc{S}) = \avg{\mc{G}(\mathrm{proj}_A(\mc{S}))} = \avg{\{\mathrm{proj}_A(g_1), \mathrm{proj}_A(g_2), \ldots, \mathrm{proj}_A(g_{m_A})\}}, \text{ where } g_{j} \in \mc{G}(\mc{S}).
}
We have $\forall m_A < i \le m, \ \exists u\in (\mathbb{F}_2)^{m_A}$  such that
\env{align}{
    \mathrm{proj}_A(g_i) = \prod_{j=1}^{m_A} \(\mathrm{proj}_A(g_j)\)^{u_j} 
}
for which
\env{align}{
    \(\mathsf{K}_A\)_{ik} = \sum_{j=1}^{m_A} u_j \(\mathsf{K}_A\)_{jk},
    \quad
    \(\mathsf{K}_A\)_{ki} = \sum_{j=1}^{m_A} u_j \(\mathsf{K}_A\)_{kj}. 
}
Using these, we can always perform a change of basis, and assume without loss of generality that
\env{align}{
\label{eq:triviality_on_A}
    \forall m_A < i \le m, \  
    \mathrm{proj}_A(g_i) = \mathbbm{1}_A.
}


We define the following $m_A \times m_A$ matrix
\env{align}{
    \(\widetilde{\mathsf{K}}_A\)_{ij}
    = \env{cases}{
        0, \text{ if } \mathrm{proj}_A(g_i) \cdot \mathrm{proj}_A(g_j) = + \mathrm{proj}_A(g_j) \cdot \mathrm{proj}_A(g_i) \\
        1, \text{ if } \mathrm{proj}_A(g_i) \cdot \mathrm{proj}_A(g_j) = - \mathrm{proj}_A(g_j) \cdot \mathrm{proj}_A(g_i)
    }
    %\text{ for } 1 \le i, j \le m_A.
}
for $1 \le i, j \le m_A$.
It is the upper-left $m_A \times m_A$ submatrix of $\mathsf{K}_A$.
As shown above, rows $m_A + 1 \ldots m$ and columns $m_A + 1 \ldots m$ of $\mathsf{K}_A$ are linearly dependent on rows $1 \ldots m_A$ and columns $1 \ldots m_A$, and can be eliminated, %. using Gauss elimination
without changing the rank.
We thus have
\env{align}{
    \dim \mathrm{Im}(\mathsf{K}_A)
    =
    \dim \mathrm{Im}(\widetilde{\mathsf{K}}_A).
}

Next, consider the center subgroup of $\mathrm{proj}_A(\mc{S})$,
\env{align}{
    Z(\mathrm{proj}_A(\mc{S})) \coloneqq \{g \in \mathrm{proj}_A(\mc{S}) \ |\ gh = hg \text{ for all } h \in \mathrm{proj}_A(\mc{S})\}.
}
Without loss of generality, let
\env{align}{
    Z(\mathrm{proj}_A(\mc{S}))
    = \avg{ \{\mathrm{proj}_A(g_1), \ldots, \mathrm{proj}_A(g_{\mu_A})\} } \text{ where } \mu_A \le m_A, \quad g_j \in \mc{G}(\mc{S}).
}
By definition, the first $\mu_A$ columns and rows of $\widetilde{\mathsf{K}}_A$ are zero, thus do not contribute to $\dim \mathrm{Im}(\widetilde{\mathsf{K}}_A)$.
%With further considerations
By induction one can show that $\widetilde{\mathsf{K}}_A$ can be brought into the following ``canonical form'' with congruence transformations~\cite{kim_two_2008},
\env{align}{
    \label{eq:KA_canonical}
    \widetilde{\mathsf{K}}_A = \env{pmatrix}{
        0_{\mu_A \times \mu_A} & 0_{\mu_A \times k_A} & 0_{\mu_A \times k_A} \\
        0_{k_A \times \mu_A} & 0_{k_A \times k_A} & \mathbbm{1}_{k_A \times k_A} \\
        0_{k_A \times \mu_A} & \mathbbm{1}_{k_A \times k_A} & 0_{k_A \times k_A}
    },
}
where $k_A$ is an integer, and $\dim \mathrm{Im}(\widetilde{\mathsf{K}}_A) = 2k_A$.
We then have
\env{align}{
    m_A =&\ \mu_A + 2k_A \nn
    \Leftrightarrow\quad 
    \dim \mathrm{proj}_A (\mc{S}) =&\ \dim Z(\mathrm{proj}_A (\mc{S})) + \dim \mathrm{Im}(\mathsf{K}_A),
}
and 
\env{align}{
    N_A(\rho_{A \cup B}) = \frac{\ln 2}{2} \dim \mathrm{Im}(\mathsf{K}_A)
    % \nn
    % =& \frac{\ln 2}{2} \dim \frac{\mathrm{proj}_A}{Z(\mathrm{proj}_A (\mc{S}))} \nn
    % =& \frac{\ln 2}{2} \log_2 \lv \frac{\mathrm{proj}_A}{Z(\mathrm{proj}_A (\mc{S}))} \rv \nn
    = \frac{1}{2} \ln \lv \frac{\mathrm{proj}_A(\mc{S})}{Z(\mathrm{proj}_A (\mc{S}))} \rv.
}
% {\blue 
% The center subgroup $Z(\mathrm{proj}_A(\mc{S}))$ defines a (possibly mixed) stabilizer state on $A$, while $\{\mathrm{proj}_A (g_{\mu_A + 1 \ldots \mu_A + k_A}) \}$ are its ``logical $X$-operators'', and $\{\mathrm{proj}_A (g_{\mu_A + k_A + 1 \ldots \mu_A + 2k_A= m_A}) \}$ are its ``logical $Z$-operators''~\cite{lyd2007capillary_qecc}.
% }




\subsection{Bounding the EN with entanglement entropies}

It is now clear that in the canonical basis of Eq.~\eqref{eq:KA_canonical},
\env{align}{
    \{\mathrm{proj}_A (g_1), \ldots, \mathrm{proj}_A (g_{\mu_A}) \} \cup \{\mathrm{proj}_A (g_{\mu_A + 1}), \ldots, \mathrm{proj}_A (g_{\mu_A + k_A}) \}
}
is a linearly independent, mutually commuting set of Pauli strings on $A$.
Thus we have
\env{align}{
    \mu_A + k_A \le |A|,
}
thus
\env{align}{
    (\ln 2)^{-1} N_A(\rho_{A \cup B}) = k_A = m_A - (\mu_A + k_A)
    \ge  m_A - |A|
    = (\ln 2)^{-1} \(S_{\rm vN}(\rho_{B}) - S_{\rm vN}(\rho_{A \cup B}) \).
}
%\TZ{The last equality is confusing. Is $S_{\rm vN}(\rho_{Q})  =0 $, since $Q$ is the total (purified) system?
%I think it should be $\ge$: $m_A - |A| = S_A \ge S_{AC} - S_C = S_{\bar{A}} - S_{A \bar{A}} $}
{Here, we recall that~\cite{Fattal2004stabilizer}
$S_{\rm vN}(\rho_{B}) = |B| - (m - m_A)$, and $S_{\rm vN}(\rho_{A \cup B}) = |{A \cup B}| - m$.}
On the other hand, consider the following set of Pauli strings on $B$,
\env{align}{
    \{\mathrm{proj}_{B} (g_{m_A + 1}),
    \mathrm{proj}_{B} (g_{m_A + 2}),
    \ldots,
    \mathrm{proj}_{B} (g_m) \}
    \cup \{\mathrm{proj}_{B} (g_{\mu_A + 1}),
    \ldots,
    \mathrm{proj}_{B} (g_{\mu_A + k_A})
    \}.
}
Using Eq.~\eqref{eq:triviality_on_A}, one can see that it is a linearly independent, mutually commuting set of Pauli strings on $B$.\footnote{
They are obviously commuting.
The linear independence is perhaps less obvious.
Let us prove by contradiction.
Suppose the product of some of these is $\mathbbm{1}_{B}$.
If this product involves some $\mathrm{proj}_{B} (g_{\mu_A + j}) (1 \le j \le k_A)$, then $\mathrm{proj}_{B} (g_{\mu_A + j})$ cannot possibly anticommute with $\mathrm{proj}_{B} (g_{\mu_A + j + k_A})$, which it must.
Thus the product must involve only $\{
    \mathrm{proj}_{B} (g_{m_A + 1}),
    \mathrm{proj}_{B} (g_{m_A + 2}),
    \ldots,
    \mathrm{proj}_{B} (g_m)\}$.
But based on Eq.~\eqref{eq:triviality_on_A}, linear dependence among these would imply linear dependence of $\{
    g_{m_A + 1},
    g_{m_A + 2},
    \ldots,
    g_m\}$, which cannot be the case either.
}
Thus
\env{align}{
    m-m_A + k_A \le |B| = |{A \cup B}| - |A|,
}
or equivalently
\env{align}{
    (\ln 2)^{-1} N_A(\rho_{A \cup B}) = k_A  \le m_A + |{A \cup B}| - |A| - m = (\ln 2)^{-1} S_{\rm vN}(\rho_{B}).
}


Therefore
\env{align}{
    \label{eq:A38}
    S_{\rm vN}(\rho_{B}) - S_{\rm vN}(\rho_{A \cup B}) \le N_A(\rho_{A \cup B}) \le S_{\rm vN}(\rho_{B}).
}
Since $ N_A(\rho_{A \cup B}) =  N_{B}(\rho_{A \cup B})$, we have
\env{align}{
    \label{eq:A39}
    & \max\{ S_{\rm vN}(\rho_{B}), S_{\rm vN}(\rho_{A}) \} - S_{\rm vN}(\rho_{A \cup B})
    \le N_A(\rho_{A \cup B})
    \le
    \min\{ S_{\rm vN}(\rho_{B}), S_{\rm vN}(\rho_{A}) \}.
}
In the case of a global pure state, $S_{\rm vN}(\rho_{A \cup B}) = 0$, and
\env{align}{
    N_A(\rho_{A \cup B}) = S_{\rm vN}(\rho_{B}) = S_{\rm vN}(\rho_{A}).
}
This result can be also obtained from the general equality between $N_A(\rho_{A \cup B})$ and $S^{1/2}(\rho_A)$ (i.e. the $\frac{1}{2}$-th R\'{e}nyi entropy of $\rho_A$) when $\rho_{A \cup B}$ is pure, and the fact that stabilizer states have flat entanglement spectra.
The identification between the negativity and entanglement entropy does not hold for mixed states in general, for in general
\env{align}{
    S_{\rm vN}(\rho_{B}) \neq S_{\rm vN}(\rho_{A})
}
while we always have
\env{align}{
    N_A(\rho_{A \cup B}) = N_{B}(\rho_{A \cup B}).
}


% We also have
% %Observe that 
% \env{align}{
% \mathrm{Ker}\ \mathrm{proj}_{\ovl{A}}(\mc{S}) \subseteq Z(\mathrm{proj}_{A}(\mc{S})),
% }
% and~\cite{li2007capillary_qecc}
% \env{align}{
% \frac{
%     Z(\mathrm{proj}_{A}(\mc{S}))
% }{
%     \mathrm{Ker}\ \mathrm{proj}_{\ovl{A}}(\mc{S})
% }
% \subseteq
% \mc{L}_A
% \coloneqq
% \frac{\ld g \in \mc{C}(\mc{S}) \ |\  \mathrm{proj}_{\ovl{A}}(g) \in \mathrm{proj}_{\ovl{A}}(\mc{S}) \rd} {\mc{S}},
% }
% so that
% \env{align}{
%     0 \le
%     \dim
%     Z(\mathrm{proj}_{A}(\mc{S}))
%     -
%     \dim
%     \mathrm{Ker}\ \mathrm{proj}_{\ovl{A}}(\mc{S})
%     \le
%     \dim \mc{L}_A = I_{A, R}.
% }
% This leads to a weaker bound on $N_A(\rho_Q)$ than those above, using results in the next subsection,
% \env{align}{
%     0 \le \frac{1}{2} I_{A, \ovl{A}} - N_A(\rho_Q) \le \frac{1}{2} I_{A, R}.
% }


\subsection{Bounding the EN with mutual information}

We compute the mutual information between $A$ and $B$,
\env{align}{
    &  (\ln 2)^{-1} I_{A, B} (\rho_{A \cup B}) \nn
    =&\ S_{\rm vN}(\rho_A) + S_{\rm vN}(\rho_{B}) - S_{\rm vN}(\rho_{A \cup B}) \nn
    =&\ (|A| - \dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S}) )
    + (|B| - \dim \mathrm{Ker}\, \mathrm{proj}_{A} (\mc{S}) ) - (|{A \cup B}| - m) \nn
    =&\, \dim \mc{S} - \dim \mathrm{Ker}\, \mathrm{proj}_{B} (\mc{S}) - \dim \mathrm{Ker}\, \mathrm{proj}_{A}(\mc{S}) \nn
    =&\, \dim \mathrm{proj}_A(\mc{S})  - \dim \mathrm{Ker}\, \mathrm{proj}_{B} (\mc{S}),
}
thus, using  $\mathrm{Ker}\ \mathrm{proj}_{B}(\mc{S}) \subseteq Z(\mathrm{proj}_{A}(\mc{S}))$,
\env{align}{
    & (\ln 2)^{-1} \(2 N_A(\rho_{A \cup B}) \) = \dim \mathrm{proj}_A(S) - \dim Z(\mathrm{proj}_A(S)) \nn
    \le& \dim \mathrm{proj}_A(\mc{S})  - \dim \mathrm{Ker}\, \mathrm{proj}_{B} (\mc{S}) = (\ln 2)^{-1} I_{A, B}(\rho_{A \cup B}),
}
or
\env{align}{
     N_A(\rho_{A \cup B}) \le \frac{1}{2} I_{A, B}(\rho_{A \cup B}).
}

We may upper bound their difference using the following observation~\cite{li2007capillary_qecc}
\env{align}{
\frac{
    Z(\mathrm{proj}_{A}(\mc{S}))
}{
    \mathrm{Ker}\ \mathrm{proj}_{B}(\mc{S})
}
\subseteq
\mc{L}_A
\coloneqq
\frac{\ld g \in \mc{C}(\mc{S}) \ |\  \mathrm{proj}_{B}(g) \in \mathrm{proj}_{B}(\mc{S}) \rd} {\mc{S}},
}
so that
\env{align}{
    0 \le
    \dim
    Z(\mathrm{proj}_{A}(\mc{S}))
    -
    \dim
    \mathrm{Ker}\ \mathrm{proj}_{B}(\mc{S})
    \le
    \dim \mc{L}_A = (\ln 2)^{-1} I_{A, C},
}
where $C$ is a purification of ${A \cup B}$, and 
\env{align}{
    I_{A,C} = S_{\rm vN}(\rho_A) + S_{\rm vN}(\rho_C) - S_{\rm vN}(\rho_{A\cup C}) = S_{\rm vN}(\rho_A) + S_{\rm vN}(\rho_{A \cup B}) - S_{\rm vN}(\rho_{B}).
}
Thus\footnote{This result maybe alternatively derived as follows:
\env{align}{
    &  I_{A,C}\nn
    =& S_{\rm vN}(\rho_A) + S_{\rm vN}(\rho_{A \cup B}) - S_{\rm vN}(\rho_{B}) \nn
    =& I_{A, B}(\rho_{A \cup B}) - 2 \lz S_{\rm vN}(\rho_{B}) - S_{\rm vN}(\rho_{{A \cup B}}) \rz \nn
    \ge& I_{A, B}(\rho_{A \cup B}) - 2 N_A(\rho_{A \cup B}), \nonumber
}
making use of Eqs.~(\ref{eq:A38}, \ref{eq:A39}).
}
\env{align}{
    0 \le \frac{1}{2} I_{A, B}(\rho_{A \cup B}) - N_A(\rho_{A \cup B}) \le \frac{1}{2} I_{A, C}.
}
In particular, it implies that $\frac{1}{2} I_{A, B}(\rho_{A \cup B}) = N_A(\rho_{A \cup B})$ when the subsystem $A$ decouples from the environment ($I_{A,C} = 0$).



\subsection{A motivating example of the structure theorem}

%-----------------------------
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{_figs/stabilizer.png}
\caption{An example of a bipartite mixed stabilizer state.
Here we have $|{A \cup B}| = 13$ lattice sites, where $|A| = 7$ and $|B| = 6$.
There are $m = 9$ stabilizers in the basis of the stabilizer group, represented by each row of $|{A \cup B}|$ squares.
Blue squares represent local Pauli $Z$ operators, red squares represent local Pauli $X$ operators, and white or gray squares represent identity operators.
Stabilizers in this basis can be classified into four sets, as detailed in Eq.~\eqref{eq:A50}.
When a stabilizer is supported nontrivially only on $A$ or $B$, they are called ``local'', and we can disregard their (trivial) content on the other subsystem (represented with gray color).
}
    \label{fig:stabilizer}
\end{figure*}
%-----------------------------

We illustrate our reasoning so far with an example, shown in Fig.~\ref{fig:stabilizer}.
This simple example represents a general pattern: with local Clifford unitaries on $A$ and $B$, we can always obtain the following ``canonical'' basis of the stabilizer group:
\env{align}{
\label{eq:A50}
    \mc{G}(\mc{S}) =& \{2 k_A \text{ stabilizers contributing to } k_A \text{ EPR pairs across $A$ and $B$}\} \nn
    &\quad \cup
    \{
    \gamma = \mu_A - \dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S}) 
    =
    \mu_{B} - \dim \mathrm{Ker}\, \mathrm{proj}_{A}(\mc{S}) \text{ ``classical'' stabilizers across $A$ and $B$}
    \} \nn
    &\quad \cup
    \{
    \dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S}) \text{ local stabilizers on $A$}
    \} \nn
    &\quad \cup
    \{
    \dim \mathrm{Ker}\, \mathrm{proj}_{{A}}(\mc{S}) \text{ local stabilizers on $B$}
    \}.
}
Here,
\env{itemize}{
\item
The first set of $2k_A$ stabilizers are those contributing to the nonzero entries of $\mathsf{K}_A$ (they pairwise anticommute when restricted to $A$ or $B$);
\item
The second set of $\gamma$ ``classical'' stabilizers and the third set of $\dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S})$ local stabilizers together generate $Z(\mathrm{proj}_{A}(\mc{S}))$; 
\item
The first three sets altogether generate $\mathrm{proj}_{A}(\mc{S})$.
}

The ``classical'' stabilizers take the form of $Z_i Z_j$, with $i \in A$ and $j \in B$, for which a stabilizer of the form $X_i X_j$ -- that anticommutes with it when restricted to either $A$ or $B$ -- is \emph{absent}.
They introduce classical correlations, and contribute to the mutual information but not the negativity,
\env{align}{
    \frac{1}{2}I_{A,B}(\rho_{A \cup B}) =&\, \(k_A + \frac{\gamma}{2}\) \ln 2, \\
    N_A(\rho_{A \cup B}) =&\, k_A \ln 2.
}
Upon the introduction of a ``reference system'' $C$ that purifies ${A \cup B}$, each of the $\gamma$ classical stabilizers extends to a tripartite GHZ state on $A$, $B$, and $C$.
With further considerations along these lines, one can obtain the ``structure theorem'' in Eq.~\eqref{eq:structural_thm}, with the following identifications
\env{align}{
    %A \to A, \quad B \to B, \quad C \to C, \\
    k_A = k_B \to e_{AB}, \quad \gamma \to g_{ABC}.
}
The structure theorem can be used to check the inequalities derived above.

==> app_EN_stab_v2.tex <==
\section{Properties of entanglement negativity (EN) of stabilizer states\label{app:EN_stab}}

\subsection{Computing EN from the commuting matrix $\mathsf{K}_A$}

Let $A$ and $B$ be two mutually exclusive sets of qubits. % of a qubit system.
Let $\mc{S}$ be a stablizer group on $A \cup B$, i.e. an abelian subgroup of the Pauli group $\mc{P}(A \cup B)$.
Let $\mc{G}(\mc{S})$ be a linearly independent generating set (the basis) of $\mc{S}$,
\begin{align}
\mc{G}(\mc{S}) =&\, \{g_1, \ldots g_{|\mc{G}(\mc{S})|} \}, \\
    \mc{S} =&\, \avg{\mc{G}(\mc{S})}
\end{align}
The dimension of $\mc{S}$ is the %number of linearly independent generators in the generating set
size of $\mc{G}(\mc{S})$, which we denote as 
\begin{equation}
\dim \mc{S} = \lv \mc{G}(\mc{S}) \rv = \log_2 \lv \mc{S} \rv.
\end{equation}
We henceforth call this number $m = \dim \mc{S}$. In general $m$ is less than or equal to the total number of the qubits in the system. The subgroup $\mc{S}$ defines the following physical density matrix on ${A \cup B}$,
\begin{align}
\rho_{A \cup B}= \frac{1}{2^{|{A \cup B}|}} \sum_{g \in \mc{S}} g.
\end{align}

The following maps are useful for the bipartition $(A,B)$ of $A \cup B$. 
\begin{itemize}
\item The ``restriction'' (or projection) on $A$:
\begin{align}
  \mathrm{proj}_A : \hspace{.3in} \mc{P}(A \cup B) \quad \to&\quad \mc{P}(A) \nn
  g_A \otimes g_B \quad \mapsto&\quad g_A
\end{align}
and similarly for $B$. 

The restriction map is a group homeomorphism, hence
\begin{equation}
\frac{\mc{S}}{\mathrm{Ker} (\text{proj}_A   )} = %\text{Im}
\text{proj}_A (\mc{S})
\end{equation}
and
\begin{equation}
m = \dim \mc{S} = \dim \mathrm{Ker} (\mathrm{proj}_A  ) + \dim \text{proj}_A (\mc{S}) %\text{Im}  (\mathrm{proj}_A  ) 
\end{equation}
According to Ref.~\cite{Fattal2004stabilizer}, 
\begin{equation}
\label{eq:S_A_B_AB}
\begin{aligned}
  %\frac{S_A}{\ln 2} 
  (\ln 2)^{-1} S_A &= |A| -  \dim \mathrm{Ker} (\mathrm{proj}_B  ) \\
  %\frac{S_B}{\ln 2} 
  (\ln 2)^{-1} S_B 
  &= |B| -  \dim \mathrm{Ker} (\mathrm{proj}_A  )\\
  %\frac{S_{AB}}{\ln 2} 
  (\ln 2)^{-1} S_{A \cup B}
  & = |A| + |B| - m. 
\end{aligned}
\end{equation}
Namely, the entanglement of a region is the length of the region minus the number of generators exclusively acting on that region. 

%To probe negativity, we define

\item The ``partial transpose'' on $A$:
\begin{align}
\Gamma_A : \hspace{.3in} \mc{P}(A \cup B) \quad \to&\quad \mc{P}(A \cup B) \nn
    g_A \otimes g_B \quad \mapsto&\quad (g_A)^\mathsf{T} \otimes g_B
\end{align}

Here $\mathsf{T}$ denotes the matrix transposition, say in the computational basis where
\begin{align}
X = \env{pmatrix}{
        0 & +1\\
        +1 & 0
    }, \quad 
    Y = \env{pmatrix}{
        0 & -i\\
        +i & 0
    }, \quad 
    Z = \env{pmatrix}{
        +1 & 0\\
        0 & -1
    }.
\end{align}

The partial transpose of $\rho_{A \cup B}$ is 
\begin{align}
\rho_{A \cup B}^{\Gamma_A} = \frac{1}{2^{|{A \cup B}|}} \sum_{g \in \mc{S}} g^{\Gamma_A}
\end{align}

\end{itemize}

Since $X^\mathsf{T} = X$, $Z^\mathsf{T} = Z$, while $Y^\mathsf{T} = -Y$, the partial transpose introduces a sign function $\text{sgn}_A(g) \coloneqq (-1)^{\#Y_A(g)}$ on $g \in \mc{P}({A \cup B})$, where $\#Y_A(g)$ counts the number of $Y$ factors in $\mathrm{proj}_A(g)$,
\env{align}{
    g^{\Gamma_A} = (-1)^{\#Y_A(g)} g = x_A(g) \cdot g.
}

We define another sign function $\mathrm{sgn}_A (g, h) \in \{-1, +1\}$ acting on two elements
\env{align}{
    \mathrm{proj}_A(g) \cdot \mathrm{proj}_A(h) = \mathrm{sgn}_A(g, h)\,  \mathrm{proj}_A(h) \cdot \mathrm{proj}_A(g).
}
A key observation is the following ``cocycle condition'', that can be explicitly verified:
\env{align}{
    x_A(g) x_A(h)  = \mathrm{sgn}_A (g, h) x_A(gh).
}

Let us also define the following $m \times m$ ``commuting matrix'',
\env{align}{
    \(\mathsf{K}_A\)_{ij} = \env{cases}{
        0, \text{ if } \mathrm{sgn}_A (g_i, g_j) = +1 \\
        %[\mathrm{proj}_A(g_i), \mathrm{proj}_A(g_j)]= 0 \\
        1, \text{ if } \mathrm{sgn}_A (g_i, g_j) = -1
        %\{\mathrm{proj}_A(g_i), \mathrm{proj}_A(g_j) \}  = 0
    },
    %\text{ for } 1 \le i, j \le m,
}
for $1 \le i, j \le m$,
where the $g_i$'s on the RHS are elements of $\mc{G}(\mc{S})$. Elementary transformations of the basis such as $g_1 \rightarrow g_1 g_2$ induces row and column transformations on $\mathsf{K}_A$, where additions and multiplications are understood over the binary field $\mathbb{F}_2$.
Hence $\mathsf{K}_A$ is a symmetric matrix over $\mathbb{F}_2$ with zero diagonal entries. 

Using the binary vector representation of $g \in \mc{S}$
\begin{equation}
g \coloneqq g^u = \prod_{j = 1}^m g_j^{u_j},  \text{ where } u \in \{0, 1\}^{m} = \(\mathbb{F}_2\)^m, g_j \in \mc{G}(\mc{S})
\end{equation}
we have 
\env{align}{
    \mathrm{sgn}_A(g^u, g^v) = (-1)^{\avg{u, \mathsf{K}_A v}}.
}

Next we show $\( \rho_{A \cup B}^{\Gamma_A} \)^2 $ is a projector. 
\env{align}{
    & \( \rho_{A \cup B}^{\Gamma_A} \)^2 
    = 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} g^{\Gamma_A} h^{\Gamma_A} 
    = 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} \text{sgn}_A(g) \text{sgn}_A(h) \cdot gh \nn
    =& 
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} \text{sgn}_A(g) \text{sgn}_A(gh) \cdot h 
    =
    \frac{1}{2^{2|{A \cup B}|}} \sum_{g, h \in \mc{S}} \mathrm{sgn}_A (g, h) \text{sgn}_A(h) \cdot h \\
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{u, v \in \(\mathbb{F}_2\)^m} \mathrm{sgn}_A (g^u, g^v) \text{sgn}_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{v \in \(\mathbb{F}_2\)^m} \( \sum_{u \in \(\mathbb{F}_2\)^m} (-1)^{\avg{u, \mathsf{K}_A v}} \) \text{sgn}_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|}} \sum_{v \in \(\mathbb{F}_2\)^m} 2^m \cdot \delta(\mathsf{K}_A v, \mathbf{0}) \cdot \text{sgn}_A(g^v) \cdot g^v \nn
    =&
    \frac{1}{2^{2|{A \cup B}|-m}} \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)} \text{sgn}_A(g^v) \cdot g^v,
}
\env{align}{
    & \( \rho_{A \cup B}^{\Gamma_A} \)^4 
    =
    \lz
    \frac{1}{2^{2|{A \cup B}|-m}} \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)} \text{sgn}_A(g^v) \cdot g^v
    \rz^2 
    =
    \frac{1}{2^{4|{A \cup B}|-2m}} \sum_{u, v \in \mathrm{Ker}(\mathsf{K}_A)} \text{sgn}_A(g^u) \text{sgn}_A(g^v) \cdot g^u g^v
    \nn
    =&
    \frac{1}{2^{4|{A \cup B}|-2m}} \sum_{u, v \in \mathrm{Ker}(\mathsf{K}_A)} (-1)^{\avg{u, \mathsf{K}_A(v)}} \text{sgn}_A(g^{u+v})  \cdot g^{u+v}
    =
    \frac{1}{2^{4|{A \cup B}|-2m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv \sum_{v \in \mathrm{Ker}(\mathsf{K}_A)}  \text{sgn}_A(g^{v})  \cdot g^{v}
    \nn
    =&
    \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv \( \rho_{A \cup B}^{\Gamma_A} \)^2.
}
Thus,
\env{align}{
    %& (\ln 2)^{-1} \mc{N}(\rho) \nn
    & (\ln 2)^{-1} N_A(\rho_{A \cup B}) 
    = \lim_{n\to \frac{1}{2}} \log_2 \mathrm{Tr} \( \rho_{A \cup B}^{\Gamma_A} \)^{2n}
    = \lim_{n\to \frac{1}{2}} \log_2 \ld
    \( \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv\)^{n-1}
    \mathrm{Tr} \( \rho_{A \cup B}^{\Gamma_A} \)^2
    \rd \nn
    =& \lim_{n\to \frac{1}{2}} \log_2 \ld
    \( \frac{1}{2^{2|{A \cup B}|-m}} \lv \mathrm{Ker}(\mathsf{K}_A) \rv\)^{n-1}
    \frac{1}{2^{|{A \cup B}|-m}}
    \rd 
    = \log_2 \( \frac{2^m}{\lv \mathrm{Ker}(\mathsf{K}_A) \rv}\)^{1/2} \nn
    =&\,
    \frac{1}{2} \lz m - \dim \mathrm{Ker}(\mathsf{K}_A) \rz 
    % =\,
    % \frac{1}{2} \dim \mathrm{Im}(\mathsf{K}_A). % \nn
    =\,
    \frac{1}{2} \mathrm{rank}(\mathsf{K}_A).
}

The generators are commutative on $A \cup B$. So if they (anti)commute on $A$, so do they in $B$. This means $\mathsf{K}_A = \mathsf{K}_B$ and 
\env{align}{
N_A(\rho_{A \cup B}) = N_B(\rho_{A \cup B}) \equiv N_{A,B}.
}
This is indeed consistent with
\env{align}{
    \(\rho_{A \cup B}^{\Gamma_A}\)^{\mathsf{T}} = \rho_{A \cup B}^{\Gamma_{B}}.
}



\subsection{The structure of the commuting matrix $\mathsf{K}_A$}
The commuting matrix $\mathsf{K}_A$ is a symmetric matrix over $\mathbb{F}_2$ with all diagonal entries being zero. The linear change of basis (generators) induces a congruent transformation on matrix $\mathsf{K}_A$, which can be reduced to a canonical form
\begin{equation}
\label{eq:K_struct}
\input{K_struct}
\end{equation}

The $m$ generators are classified into four groups. The first $2k_A$ are $k_A$ pairs of anti-commuting generators. They are directly related to the negativity, 
\begin{equation}
%\frac{N_A}{\ln 2}
(\ln 2)^{-1} N_{A, B} = \frac{1}{2} \text{rank}( \mathsf{K}_A ) = k_A 
\end{equation}

There are $m_A$ linearly independent generators in $\text{proj}_A(\mc{S})$. These are listed as the first $m_A$ generators in $\mathsf{K}_A$. The maximal abelian subgroup in $\text{proj}_A(\mc{S})$ has $m_A - 2k_A = \mu _A$ generators. Hence the dimension of the center is 
\begin{equation}
\dim Z ( \text{proj}_A(\mc{S}) ) = \mu_A  
\end{equation}
In general $g \in \mathrm{Ker}\, \text{proj}_B$ is exclusively on $A$, which means it should commute with all the other generators in $A$, hence %$g \in Z ( \text{Im} (\text{proj}_A ) )$. We have
\begin{equation}
\mathrm{Ker} \, \text{proj}_B \subseteq Z ( \text{proj}_A(\mc{S}) )
\end{equation}
and
\begin{equation}
\begin{aligned}
  \dim \mathrm{Ker}\, \text{proj}_B &\le \dim Z ( \text{proj}_A(\mc{S}) ) \\
  &= \mu_A = m_A - 2k_A 
\end{aligned}
\end{equation}
Finally the dimension suggests
\begin{equation}
m - m_A = m - \dim \text{proj}_A(\mc{S}) = \dim \mathrm{Ker}\, \text{proj}_A
\end{equation}
In fact, we can use the first $m_A$ generators to reduce the $A$ part of the last $m - m_A$ generators to be identity, and these last $m - m_A$ stabilizers generate $\mathrm{Ker}\, \text{proj}_A$. 

We derive another important inequality
\begin{equation}
m_A - k_A \le |A| 
\end{equation}
This is established by taking the $(k_A + 1)$-th to the $m_A$-th generators (corresponds to the red box in the $\mathsf{K}_A$ matrix in Eq.~\eqref{eq:K_struct}). They are linearly independent on $A$ (for they are among the first $m_A$ generators) and mutually commutative (zero entries in the commuting matrix). Hence the number is less than the number of qubits in $A$.


\subsection{Bounds of EN}

We derive bounds of EN from entanglement and mutual information through reducing to the inequalities 
\begin{equation}
\dim \mathrm{Ker}\, \text{proj}_B \le m_A - 2k_A 
\end{equation}
and 
\begin{equation}
m_A - k_A \le |A| 
\end{equation}
derived from the structure of the $\mathsf{K}_A$ matrix in the previous section. 


{\bf Bounds from entanglement}:
\begin{equation}
\label{eq:neg_ineq_s}
\max ( S_A, S_B ) - S_{A \cup B} \le N_{A, B}  \le \min ( S_A, S_B ).
\end{equation}

{\it Proof}: We prove 
\begin{equation}
S_B - S_{A \cup B}  \le  N_{A, B}  \le S_A
\end{equation}
then interchange $A$ and $B$ to obtain Eq.~\eqref{eq:neg_ineq_s}. 


$S_B - S_{A \cup B}  \le  N_{A, B}$: using expressions of entanglement in Eq.~\eqref{eq:S_A_B_AB}: 
\begin{equation}
\begin{aligned}
\Leftrightarrow&   \quad |B| - \dim \mathrm{Ker}\, \text{proj}_A - ( |A|+|B| - m )  \le k_A   \quad \Leftrightarrow  \quad  \dim \text{proj}_A(\mc{S}) - |A| \le k_A \\
\Leftrightarrow& \quad  m_A- k_A \le |A|; 
\end{aligned}
\end{equation}

$N_{A, B}  \le S_A$: 
\begin{equation}
\label{eq:neg_less_s}
\Leftrightarrow \quad k_A  \le |A| - \dim \mathrm{Ker}\, \text{proj}_B \quad \Leftrightarrow \quad  k_A  + \dim \mathrm{Ker}\, \text{proj}_B \le |A|. 
\end{equation}
From $\dim \mathrm{Ker}\, \text{proj}_B \le m - 2k_A $, we have
\begin{equation}
k_A + \dim \mathrm{Ker} \, \text{proj}_B  \le m - k_A \le |A|. 
\end{equation}


{\bf Bounds of EN from mutual information}: 

We purify the state $AB$ into $ABC$, then 

\begin{equation}
\frac{1}{2}( I_{A,B} - I_{A,C} ) \le N_{A,B} \le \frac{1}{2} I_{A,B} 
\end{equation}
{\it Proof}:

{\bf LHS}: 
\begin{equation}
I_{A,C} = S_A + S_{AB} - S_B, \quad I_{A,B} = S_A + S_B - S_{AB} \implies \frac{1}{2}( I_{A,B} - I_{A,C} ) = S_B - S_{AB} \le N_{A,B}.
\end{equation}
This has been established in Eq.~\eqref{eq:neg_ineq_s}

{\bf RHS}: using expressions of entanglement in Eq.~\eqref{eq:S_A_B_AB}
\begin{equation}
\begin{aligned}
&\Leftrightarrow \quad 2k_A \le  m -  \dim \mathrm{Ker}\, \text{proj}_A - \dim \mathrm{Ker}\, \text{proj}_B \\
&\Leftrightarrow \quad 2k_A \le \dim \text{proj}_A(\mc{S}) - \dim \mathrm{Ker}\, \text{proj}_B  \\
&\Leftrightarrow \quad \dim \mathrm{Ker}\, \text{proj}_B \le m_A - 2k_A. 
\end{aligned}
\end{equation}




\subsection{A motivating example of the structure theorem}

%-----------------------------
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{_figs/stabilizer.png}
\caption{An example of a bipartite mixed stabilizer state.
Here we have $|{A \cup B}| = 13$ lattice sites, where $|A| = 7$ and $|B| = 6$.
There are $m = 9$ stabilizers in the basis of the stabilizer group, represented by each row of $|{A \cup B}|$ squares.
Blue squares represent local Pauli $Z$ operators, red squares represent local Pauli $X$ operators, and white or gray squares represent identity operators.
Stabilizers in this basis can be classified into four sets, as detailed in Eq.~\eqref{eq:A50}.
When a stabilizer is supported nontrivially only on $A$ or $B$, they are called ``local'', and we can disregard their (trivial) content on the other subsystem (represented with gray color).
}
    \label{fig:stabilizer}
\end{figure*}
%-----------------------------

We illustrate our reasoning so far with an example, shown in Fig.~\ref{fig:stabilizer}.
This simple example represents a general pattern: with local Clifford unitaries on $A$ and $B$, we can always obtain the following ``canonical'' basis of the stabilizer group:
\env{align}{
\label{eq:A50}
    \mc{G}(\mc{S}) =& \{2 k_A \text{ stabilizers contributing to } k_A \text{ EPR pairs across $A$ and $B$}\} \nn
    &\quad \cup
    \{
    \gamma = \mu_A - \dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S}) 
    =
    \mu_{B} - \dim \mathrm{Ker}\, \mathrm{proj}_{A}(\mc{S}) \text{ ``classical'' stabilizers across $A$ and $B$}
    \} \nn
    &\quad \cup
    \{
    \dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S}) \text{ local stabilizers on $A$}
    \} \nn
    &\quad \cup
    \{
    \dim \mathrm{Ker}\, \mathrm{proj}_{{A}}(\mc{S}) \text{ local stabilizers on $B$}
    \}.
}
Here,
\env{itemize}{
\item
The first set of $2k_A$ stabilizers are those contributing to the nonzero entries of $\mathsf{K}_A$ (they pairwise anticommute when restricted to $A$ or $B$);
\item
The second set of $\gamma$ ``classical'' stabilizers and the third set of $\dim \mathrm{Ker}\, \mathrm{proj}_{B}(\mc{S})$ local stabilizers together generate $Z(\mathrm{proj}_{A}(\mc{S}))$; 
\item
The first three sets altogether generate $\mathrm{proj}_{A}(\mc{S})$.
}

The ``classical'' stabilizers take the form of $Z_i Z_j$, with $i \in A$ and $j \in B$, for which a stabilizer of the form $X_i X_j$ -- that anticommutes with it when restricted to either $A$ or $B$ -- is \emph{absent}.
They introduce classical correlations, and contribute to the mutual information but not the negativity,
\env{align}{
    \frac{1}{2}I_{A,B}(\rho_{A \cup B}) =&\, \(k_A + \frac{\gamma}{2}\) \ln 2, \\
    N_A(\rho_{A \cup B}) =&\, k_A \ln 2.
}
Upon the introduction of a ``reference system'' $C$ that purifies ${A \cup B}$, each of the $\gamma$ classical stabilizers extends to a tripartite GHZ state on $A$, $B$, and $C$.
With further considerations along these lines, one can obtain the ``structure theorem'' in Eq.~\eqref{eq:structural_thm}, with the following identifications
\env{align}{
    %A \to A, \quad B \to B, \quad C \to C, \\
    k_A = k_B \to e_{AB}, \quad \gamma \to g_{ABC}.
}
The structure theorem can be used to check the inequalities derived above.


%%% Local Variables:
%%% TeX-master: "app"
%%% TeX-PDF-mode: t
%%% mode: latex
%%% End:

